What do online listings tell us about the housing market?

Traditional data sources for the analysis of housing markets show several limitations, that recently started to be overcome using data coming from housing sales advertisements (ads) websites. In this paper, using a large dataset of ads in Italy, we provide the first comprehensive analysis of the problems and potential of these data. The main problem is that multiple ads ("duplicates") can correspond to the same housing unit. We show that this issue is mainly caused by sellers' attempt to increase visibility of their listings. Duplicates lead to misrepresentation of the volume and composition of housing supply, but this bias can be corrected by identifying duplicates with machine learning tools. We then focus on the potential of these data. We show that the timeliness, granularity, and online nature of these data allow monitoring of housing demand, supply and liquidity, and that the (asking) prices posted on the website can be more informative than transaction prices.

==> tables/ads_tomtable.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Wed Aug  9 09:50:53 2017
\begin{table}[ht]
\centering
\begin{tabular}{cccc}
  \hline
Year & Quarter & IMM & Survey BI \\ 
  \hline
2016 & 1 & 4.6 & 7.5 \\ 
  2016 & 2 & 4.0 & 7.7 \\ 
  2016 & 3 & 4.4 & 7.9 \\ 
  2016 & 4 & 4.4 & 6.8 \\ 
  2017 & 1 & 4.8 & 6.4 \\ 
  2017 & 2 & 4.2 & 6.4 \\ 
   \hline
\end{tabular}
\caption{Time on market. Comparison between ads and the Italian housing market survey, conducted by the Bank of Italy.} 
\label{table:ads_tomtable}
\end{table}


==> tables/ads_totabsales.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Wed Aug  9 09:49:05 2017
\begin{table}[ht]
\centering
\begin{tabular}{lccc}
  \hline
City & IMM & OMI & IMM/OMI*100 \\ 
  \hline
Turin & 20263 & 12322 & 164.4 \\ 
  Genoa & 10358 & 6601 & 156.9 \\ 
  Milan & 40342 & 21909 & 184.1 \\ 
  Bologna & 7655 & 5507 & 139.0 \\ 
  Florence & 12833 & 4786 & 268.1 \\ 
  Rome & 73070 & 30173 & 242.2 \\ 
  Naples & 9764 & 6650 & 146.8 \\ 
  Palermo & 5504 & 4718 & 116.7 \\ 
   \hline
\end{tabular}
\caption{Transactions. Comparison between ads and OMI data.} 
\label{table:ads_totabsales}
\end{table}


==> tables/aggregate_regressions_pricem2.tex <==

\begin{table}[!h] \centering 
\small 
\begin{tabular}{lcc} 
\hline 
\hline \\ 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\& Average price & Liquidity \\ 
\\  & (1) & (2)\\ 
\hline \\  
  Demand$_{t-1}$ & 0.033$^{**}$ &  0.060$^{***}$ \\ 
  & (0.015) &  (0.018)  \\ 
  Demand$_{t-2}$ & 0.048$^{***}$ & 0.138$^{***}$    \\ 
  & (0.015) &  (0.018)   \\ 
  Average price$_{t-1}$ & 0.528$^{***}$ &   \\ 
  & (0.009) &   \\ 
  Liquidity$_{t-1}$ &  & 0.161$^{***}$  \\ 
  &   & (0.011)  \\
  Education & 0.917$^{***}$ & -0.321$^{***}$ \\ 
  & (0.045) & (0.052)   \\ 
  Unemployment (share) & -2.026$^{***}$ & 1.143$^{***}$  \\ 
  & (0.236) & (0.293)   \\ 
  Homeowners (share) & -0.438$^{***}$ & 0.174$^{***}$   \\ 
  & (0.036) & (0.044)   \\ 
  Foreigners (share) & -0.386$^{***}$ & 0.130$^{***}$  \\ 
  & (0.051) & (0.063)  \\ 
  Constant & 3.144$^{***}$ & -2.169$^{***}$   \\ 
  & (0.095) & (0.096)   \\ 
 \hline \\
Fixed effects & City+Time & City+Time  \\ 
Observations &  8,851 &  8,851  \\ 
\hline 
\hline \\  
\end{tabular} 
\caption{} 
  \label{} 
\end{table} 


==> tables/atipicality.tex <==
% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: ven, ott 06, 2017 - 22:21:57
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Atypicality} 
  \label{tab:atypicality} 
\begin{tabular}{@{\extracolsep{-50pt}}lD{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{1}{c}{Price per m2} & \multicolumn{1}{c}{Time on market}\\ 
\hline \\[-1.8ex] 
  Price heterogeneity & 1.133$ $(18.692) & 4.914$ $(4.914) \\ 
  Floor heterogeneity & -52.128$ $(31.700) & -3.206$ $(8.546) \\ 
  Floor area heterogeneity & -3.998$ $(23.342) & 8.695$ $(6.118) \\ 
  Rooms heterogeneity & 4.335$ $(37.742) & -0.662$ $(10.305) \\ 
  Constant & 1,662.831^{***}$ $(462.390) & 147.532^{*}$ $(89.070) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{168,073} & \multicolumn{1}{c}{53,208} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.780} & \multicolumn{1}{c}{0.235} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.778} & \multicolumn{1}{c}{0.211} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
 & \multicolumn{2}{r}{OMI micro-zone and quarter dummies. Other controls
                  include  } \\ 
 & \multicolumn{2}{r}{housing unit characteristics, and the tightness and mean price } \\ 
 & \multicolumn{2}{r}{per m2 in the neighborhood (lagged).} \\ 
\end{tabular} 
\end{table} 

==> tables/duplicates_table.tex <==
%% Table with duplicates

\begin{table}[!h]
\centering
\footnotesize
 \begin{tabular}{lccccccc}
  \hline
  & 1 & 2 & 3 & 4 & 5 & 6 & 7 or more \\
  \hline
  Number of dwellings & 730,917 & 128,194 & 39,744 & 17,795 & 9,195 & 5,624 & 13,461 \\
  Share on total \% & 77.4 & 13.6 & 4.2 & 1.9 & 0.9 & 0.6 & 1.4 \\
  \hline
 \end{tabular}
\caption{Distribution of dwellings by number of associated ads}
\label{table:distr_duplicates}
\end{table}

==> tables/dwell_liquiditytable.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Wed Aug  9 10:07:06 2017
\begin{table}[ht]
\centering
\begin{tabular}{lccccccccccc}
  \hline
Period & Sales & For sale &\multicolumn{9}{c}{Liquidity} \\ 
          &       &                    & All cities & To & Ge & Mi & Bo & Fi & Rm & Na & Pa \\   
\hline
  2016Q1 & 24655 & 205771 & 12.0 & 13.2 & 13.2 & 13.9 & 13.8 & 14.9 & 12.6 & 14.1 & 11.5 \\ 
  2016Q2 & 31618 & 208413 & 15.2 & 16.4 & 16.2 & 17.9 & 16.9 & 16.5 & 15.3 & 17.9 & 15.0 \\ 
  2016Q3 & 22647 & 187864 & 12.1 & 11.9 & 12.7 & 12.9 & 11.9 & 13.3 & 12.3 & 16.4 & 9.3 \\ 
  2016Q4 & 29689 & 199600 & 14.9 & 15.0 & 16.0 & 16.3 & 15.4 & 18.7 & 15.2 & 18.4 & 11.9 \\ 
  2017Q1 & 33260 & 199898 & 16.6 & 17.1 & 15.9 & 18.7 & 20.0 & 21.2 & 16.4 & 18.6 & 16.5 \\ 
  2017Q2 & 28272 & 195771 & 14.4 & 15.4 & 15.7 & 17.3 & 16.5 & 17.2 & 14.0 & 18.1 & 12.9 \\ 
   \hline
\end{tabular}
\caption{Transactions, supply and liquidity.} 
\label{table:dwell_liquiditytable}
\end{table}


==> tables/dwell_pricedistr.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Thu Sep 21 22:05:28 2017
\begin{table}[ht]
\centering
\begin{tabular}{lcccccccc}
  \hline
Year & 5th & 15th & 25th & 50th & 75th & 85th & 95th & Mean \\ 
  \hline
  & \multicolumn{8}{c}{Full sample}   \\
2016 & 915 & 1235 & 1500 & 2167 & 3125 & 3778 & 5143 & 2487 \\ 
  2017 & 857 & 1161 & 1417 & 2067 & 3000 & 3672 & 5053 & 2398 \\ 
\hline  
  y-o-y variation & -6.3 & -6.0 & -5.6 & -4.6 & -4.0 & -2.8 & -1.8 & -3.6 \\ 
   \hline
 & \multicolumn{8}{c}{Milan}   \\
2016 & 1667 & 2083 & 2409 & 3200 & 4400 & 5182 & 6861 & 3588 \\ 
  2017 & 1635 & 2067 & 2388 & 3192 & 4474 & 5333 & 6957 & 3617 \\ 
\hline  
  y-o-y variation & -1.9 & -0.8 & -0.9 & -0.3 & 1.7 & 2.9 & 1.4 & 0.8 \\ 
   \hline   
   & \multicolumn{8}{c}{Turin}   \\
   2016 & 863 & 1107 & 1311 & 1750 & 2316 & 2684 & 3500 & 1900 \\ 
  2017 & 824 & 1060 & 1253 & 1700 & 2256 & 2659 & 3500 & 1860 \\ 
\hline  
  y-o-y variation & -4.6 & -4.2 & -4.4 & -2.9 & -2.6 & -0.9 & 0.0 & -2.1 \\ 
  \hline
  & \multicolumn{8}{c}{Rome}   \\
  2016 & 1731 & 2222 & 2548 & 3278 & 4231 & 4900 & 6316 & 3557 \\ 
  2017 & 1627 & 2106 & 2438 & 3173 & 4133 & 4780 & 6212 & 3448 \\ 
\hline  
  y-o-y variation & -6.0 & -5.2 & -4.4 & -3.2 & -2.3 & -2.4 & -1.6 & -3.1 \\ 
   \hline
   & \multicolumn{8}{c}{Naples}   \\
   2016 & 1154 & 1532 & 1833 & 2667 & 3875 & 4600 & 6047 & 3007 \\ 
  2017 & 1078 & 1435 & 1722 & 2544 & 3750 & 4465 & 5900 & 2894 \\ 
 \hline  
  y-o-y variation & -6.6 & -6.3 & -6.1 & -4.6 & -3.2 & -2.9 & -2.4 & -3.8 \\ 
   \hline
   \hline
\end{tabular}
\caption{Evolution of the asking prices per square meter between 2016S1 and 2017S1 across several quantiles of the price distribution. In the top lines we show the aggregate dynamics, below we consider the four largest Italian cities. The dynamics are similar.} 
\label{table:dwell_pricedistr}
\end{table}


==> tables/dwell_tomtable.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Wed Aug  9 09:53:31 2017
\begin{table}[ht]
\centering
\begin{tabular}{cccc}
  \hline
Year & Quarter & IMM & Survey BI \\ 
  \hline
2016 & 1 & 7.3 & 7.5 \\ 
  2016 & 2 & 7.1 & 7.7 \\ 
  2016 & 3 & 7.7 & 7.9 \\ 
  2016 & 4 & 7.8 & 6.8 \\ 
  2017 & 1 & 8.2 & 6.4 \\ 
  2017 & 2 & 7.9 & 6.4 \\ 
   \hline
\end{tabular}
\caption{Time on market. Comparison between the housing units dataset and the Italian Housing Market Survey, conducted by the Bank of Italy.} 
\label{table:dwell_tomtable}
\end{table}


==> tables/dwell_totabsales.tex <==
% latex table generated in R 3.2.3 by xtable 1.8-2 package
% Wed Aug  9 09:52:20 2017
\begin{table}[ht]
\centering
\begin{tabular}{lccc}
  \hline
City & IMM & OMI & Coverage \\ 
  \hline
Turin & 7615 & 12322 & 61.8 \\ 
  Genoa & 4816 & 6601 & 73.0 \\ 
  Milan & 12570 & 21909 & 57.4 \\ 
  Bologna & 2866 & 5507 & 52.0 \\ 
  Florence & 4122 & 4786 & 86.1 \\ 
  Rome & 22103 & 30173 & 73.3 \\ 
  Naples & 3832 & 6650 & 57.6 \\ 
  Palermo & 2427 & 4718 & 51.4 \\ 
   \hline
\end{tabular}
\caption{Transactions. Comparison between the housing units dataset and OMI data.} 
\label{table:dwell_totabsales}
\end{table}


==> tables/hedreg_pricem2_multiple.tex <==
\begin{landscape}

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: dom, set 10, 2017 - 12:49:45
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Hedonic regression} 
  \label{tab:hedregression} 
\begin{tabular}{@{\extracolsep{-30pt}}lD{.}{.}{-3} D{.}{.}{-3} D{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & \multicolumn{3}{c}{Price per m2} \\ 
 & \multicolumn{1}{c}{Italy} & \multicolumn{1}{c}{Rome} & \multicolumn{1}{c}{Milan} \\ 
\\[-1.8ex] & \multicolumn{1}{c}{(1)} & \multicolumn{1}{c}{(2)} & \multicolumn{1}{c}{(3)}\\ 
\hline \\[-1.8ex] 
 Number of bathrooms & 154.577^{***}$ $(3.743) & 72.178^{***}$ $(8.034) & 208.084^{***}$ $(12.031) \\ 
  Floor of the apartment & 32.363^{***}$ $(0.926) & 51.505^{***}$ $(2.077) & 48.876^{***}$ $(2.338) \\ 
  Floor area [m2] & -1.281^{***}$ $(0.048) & -2.811^{***}$ $(0.102) & -0.141$ $(0.174) \\ 
  Number of rooms & -22.093^{***}$ $(2.103) & -48.384^{***}$ $(4.904) & -21.860^{***}$ $(8.086) \\ 
  Air conditioning & 106.661^{***}$ $(3.499) & 126.300^{***}$ $(7.545) & 122.863^{***}$ $(10.211) \\ 
  Balcony & -30.398^{***}$ $(3.693) & 11.483$ $(7.912) & 0.764$ $(10.935) \\ 
  Elevator & 168.574^{***}$ $(3.969) & 144.780^{***}$ $(9.708) & 223.752^{***}$ $(12.614) \\ 
  Energy class; Ref: EG; Level: AB & 360.102^{***}$ $(7.560) & 267.614^{***}$ $(18.907) & 393.328^{***}$ $(21.635) \\ 
  Energy class; Ref: EG; Level: CD & 114.052^{***}$ $(5.742) & 92.140^{***}$ $(20.624) & 135.590^{***}$ $(16.620) \\ 
  Garage; Ref: No; Level: Single & 120.817^{***}$ $(5.838) & 127.548^{***}$ $(11.158) & 108.439^{***}$ $(27.483) \\ 
  Garage; Ref: No; Level: Double & 205.992^{***}$ $(4.330) & 319.284^{***}$ $(10.700) & 149.507^{***}$ $(12.491) \\ 
  Heating type; Ref: No; Level: Centralized & 47.737^{***}$ $(10.439) & 156.469^{***}$ $(29.439) & 225.680^{**}$ $(88.304) \\ 
  Heating type; Ref: No; Level: Autonomous & 135.250^{***}$ $(9.878) & 222.994^{***}$ $(29.050) & 281.075^{***}$ $(88.417) \\ 
  Kitchen type; Ref: Kitchenette; Level: Small eat-in kitchen & -49.458^{***}$ $(5.350) & -23.742^{**}$ $(11.736) & -89.975^{***}$ $(14.268) \\ 
  Kitchen type; Ref: Kitchenette; Level: Large eat-in kitchen & -77.403^{***}$ $(4.477) & -86.146^{***}$ $(10.131) & -57.177^{***}$ $(12.522) \\ 
  Status; Ref: To renovate; Level: Good & 192.238^{***}$ $(5.661) & 164.210^{***}$ $(11.707) & 186.031^{***}$ $(16.280) \\ 
  Status; Ref: To renovate; Level: Excellent & 480.591^{***}$ $(5.874) & 462.987^{***}$ $(12.252) & 535.513^{***}$ $(16.606) \\ 
  Status; Ref: To renovate; Level: New & 610.984^{***}$ $(8.808) & 479.285^{***}$ $(21.080) & 584.823^{***}$ $(25.053) \\ 
  Terrace & 143.539^{***}$ $(3.761) & 229.414^{***}$ $(8.255) & 217.474^{***}$ $(12.834) \\ 
  Utility room & -56.913^{***}$ $(3.516) & -84.680^{***}$ $(8.234) & -77.461^{***}$ $(10.396) \\ 
  Basement & 11.039^{***}$ $(3.660) & 57.360^{***}$ $(8.388) & 24.695^{**}$ $(9.814) \\ 
  Porter & 99.019^{***}$ $(5.557) & 73.887^{***}$ $(10.685) & 62.285^{***}$ $(10.476) \\ 
  Constant & 718.810^{***}$ $(241.357) & 2,026.932^{***}$ $(724.520) & 457.625$ $(749.341) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{174,143} & \multicolumn{1}{c}{43,945} & \multicolumn{1}{c}{27,212} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.783} & \multicolumn{1}{c}{0.675} & \multicolumn{1}{c}{0.731} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.781} & \multicolumn{1}{c}{0.673} & \multicolumn{1}{c}{0.730} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
 & \multicolumn{3}{r}{OMI micro-zone and quarter dummies} \\ 
\end{tabular} 
\end{table} 
\end{landscape}


==> tables/micro_regressions.tex <==

\begin{table}[!h] \centering 
\scriptsize 
\begin{tabular}{lcccc} 
\hline 
\hline
\\ 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\ 
& Time on market & Price decrease & Price increase \\ 
 & \textit{OLS} &  \textit{logistic}  &  \textit{logistic} \\ 
 & (1) & (2)& (3) \\ 
\hline \\ 
 Relative demand & -0.599$^{***}$ &   -0.120$^{***}$ & 0.130$^{***}$ \\ 
  & (0.002) &   (0.010) & (0.036) \\ 
  Price  & -0.068$^{***}$ &  0.265$^{***}$ & -0.417$^{***}$ \\ 
  & (0.006) &  (0.015) & (0.020) \\ 
  Floor area  & 0.0003$^{***}$  & 0.0001 & 0.00004 \\ 
  & (0.00004) &  (0.0001) & (0.0003) \\ 
  Maintenance status & -0.032$^{***}$   & -0.198$^{***}$ & 0.557$^{***}$ \\ 
  & (0.002) &   (0.007) & (0.024) \\ 
  Number of rooms & 0.027$^{***}$   & -0.001 & 0.034 \\ 
  & (0.002) &   (0.006) & (0.021) \\ 
  Constant & 4.094$^{***}$   & 535.437 & 441.083 \\ 
  & (0.227)   & (505.245) & (5,861.501) \\
  OMI+Time dummies & Yes & Yes & Yes \\ 
 \hline \\ 
Observations & 201,208 &  200,000 & 200,000 \\ 
\hline 
\hline \\
\end{tabular} 
  \caption{} 
  \label{} 
\end{table} 


==> tables/regression_duplicates.tex <==
% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Aug 10, 2017 - 04:10:57 PM
\begin{table}[!htbp] \centering 
  \caption{Determinants of duplicated ads} 
  \label{table:regression_duplicates} 
\begin{tabular}{@{\extracolsep{5pt}}lccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{5}{c}{\textit{Dependent variable:}} \\ 
\cline{2-6} 
\\[-1.8ex] & \multicolumn{5}{c}{Ad is duplicated} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5)\\ 
\hline \\[-1.8ex] 
  Demand & $-$0.597$^{***}$ &  &  &  & $-$0.295$^{***}$ \\ 
  & (0.006) &  &  &  & (0.007) \\ 
  & & & & & \\ 
 Daily demand &  & $-$1.824$^{***}$ &  &  & $-$1.786$^{***}$ \\ 
  &  & (0.011) &  &  & (0.011) \\ 
  & & & & & \\ 
 Overvaluation &  &  & 0.092$^{***}$ &  & $-$0.529$^{***}$ \\ 
  &  &  & (0.024) &  & (0.044) \\ 
  & & & & & \\ 
 Hedonic overvaluation &  &  &  & 0.132$^{***}$ & $-$0.944$^{***}$ \\ 
  &  &  &  & (0.023) & (0.045) \\ 
  & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 197,860 & 197,860 & 197,860 & 197,860 & 197,860 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{5}{r}{ $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

==> tables/summary-statistics-categorical.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Wed Mar 27 19:38:21 2019
\begingroup\footnotesize
\begin{longtable}{llrr}
 \textbf{Variable} & \textbf{Levels} & $\mathbf{n}$ & $\mathbf{\%}$ \\ 
  \hline
Area territoriale & Centro & 230,246 & 32.5 \\ 
   & Nord-Ovest & 226,220 & 31.9 \\ 
   & Nord-Est & 117,498 & 16.6 \\ 
   & Sud & 76,556 & 10.8 \\ 
   & Isole & 49,451 & 7.0 \\ 
   & Missing value & 9,647 & 1.4 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Regione & Lazio & 150,025 & 21.1 \\ 
   & Lombardia & 117,262 & 16.5 \\ 
   & Piemonte & 69,445 & 9.8 \\ 
   & Emilia-Romagna & 62,181 & 8.8 \\ 
   & Toscana & 59,955 & 8.4 \\ 
   & Sicilia & 43,143 & 6.1 \\ 
   & Veneto & 42,130 & 5.9 \\ 
   & Liguria & 38,328 & 5.4 \\ 
   & Campania & 29,911 & 4.2 \\ 
   & Puglia & 27,268 & 3.8 \\ 
   & (Others) & 67,170 & 9.5 \\ 
   & Missing value & 2,800 & 0.4 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Comune & Roma & 140,854 & 19.9 \\ 
   & Milano & 71,444 & 10.1 \\ 
   & Torino & 50,725 & 7.2 \\ 
   & Genova & 30,731 & 4.3 \\ 
   & Napoli & 23,094 & 3.2 \\ 
   & Firenze & 21,363 & 3.0 \\ 
   & Palermo & 19,769 & 2.8 \\ 
   & Bologna & 17,850 & 2.5 \\ 
   & Padova & 12,727 & 1.8 \\ 
   & Bari & 10,542 & 1.5 \\ 
   & (Others) & 307,719 & 43.4 \\ 
   & Missing value & 2,800 & 0.4 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Energy class & G & 335,253 & 47.2 \\ 
   & F & 73,553 & 10.4 \\ 
   & E & 46,138 & 6.5 \\ 
   & D & 31,495 & 4.4 \\ 
   & A & 27,122 & 3.8 \\ 
   & C & 20,057 & 2.8 \\ 
   & B & 17,848 & 2.5 \\ 
   & Not available & 17,800 & 2.5 \\ 
   & Missing value & 140,352 & 19.8 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Maintenance status & Good & 268,520 & 37.8 \\ 
   & Excellent & 255,187 & 36.0 \\ 
   & To renovate & 91,644 & 12.9 \\ 
   & New & 62,931 & 8.9 \\ 
   & Missing value & 31,336 & 4.4 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Elevator & True & 389,341 & 54.9 \\ 
   & False & 320,277 & 45.1 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Kitchen type & Large eat-in kitchen & 422,560 & 59.5 \\ 
   & Kitchenette & 123,072 & 17.3 \\ 
   & Small eat-in kitchen & 91,992 & 13.0 \\ 
   & Missing value & 71,994 & 10.2 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Heating type & Autonomous & 414,933 & 58.5 \\ 
   & Centralized & 214,842 & 30.3 \\ 
   & Missing & 35,530 & 5.0 \\ 
   & Missing value & 44,313 & 6.2 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Floor & 1 & 187,730 & 26.5 \\ 
   & 2 & 120,902 & 17.0 \\ 
   & 3 & 90,051 & 12.7 \\ 
   & 0 & 88,984 & 12.5 \\ 
   & 4 & 56,920 & 8.0 \\ 
   & On multiple floors & 50,050 & 7.0 \\ 
   & 5 & 33,604 & 4.7 \\ 
   & 6 & 18,072 & 2.5 \\ 
   & 7 & 9,935 & 1.4 \\ 
   & -1 & 5,781 & 0.8 \\ 
   & (Others) & 9,226 & 1.3 \\ 
   & Missing value & 38,363 & 5.4 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Air conditioning & False & 155,361 & 21.9 \\ 
   & True & 152,067 & 21.4 \\ 
   & Missing value & 402,190 & 56.7 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Property type & Apartment & 641,735 & 90.4 \\ 
   & Villa & 67,883 & 9.6 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Balcony & True & 450,126 & 63.4 \\ 
   & False & 259,492 & 36.6 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Terrace & False & 479,280 & 67.5 \\ 
   & True & 230,338 & 32.5 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Garden type & Missing & 442,356 & 62.3 \\ 
   & Shared & 148,318 & 20.9 \\ 
   & Private & 118,944 & 16.8 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Garage & Missing & 454,323 & 64.0 \\ 
   & Double & 204,883 & 28.9 \\ 
   & Single & 50,412 & 7.1 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Porter & False & 652,497 & 92.0 \\ 
   & True & 57,121 & 8.1 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Basement & False & 442,900 & 62.4 \\ 
   & True & 266,718 & 37.6 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
Utility room & False & 502,773 & 70.8 \\ 
   & True & 206,845 & 29.1 \\ 
   \hline
 & all & 709,618 & 100.0 \\ 
   \hline
\hline
\hline
\caption{Categorical variables} 
\label{tab:summstatcleanedcat}
\end{longtable}
\endgroup



==> tables/summary-statistics-date.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Wed Mar 27 19:20:08 2019
\begingroup\footnotesize
\begin{longtable}{lrrrrrrrr}
  \hline
Variable & N & Min. & 1st Qu. & Median & Mean & 3rd Qu. & Max. & Missing \\ 
  \hline
city\_istat\_code & 709618 & 1272 & 15146 & 48017 & 43431.73 & 58091 & 110009 &   0 \\ 
  floor\_area & 703075 & 27 & 70 & 93 & 107.7543 & 125 & 500 & 6543 \\ 
  latitude & 709618 & 36.7792 & 41.8735 & 43.9165 & 43.33145 & 45.3693 & 46.5157 &   0 \\ 
  longitude & 709618 & 7.28468 & 9.21541 & 11.5986 & 11.44547 & 12.5686 & 18.3053 &   0 \\ 
  rooms & 689219 & 1 & 2 & 3 & 3.296192 & 4 & 5 & 20399 \\ 
  bathrooms & 698000 & 1 & 1 & 1 & 1.469808 & 2 & 3 & 11618 \\ 
  n\_duplicates & 709618 & 1 & 1 & 1 & 1.584505 & 2 & 99 &   0 \\ 
  timeonmarket & 703632 & 15 & 74 & 158 & 240.3546 & 300 & 1733 & 5986 \\ 
  price & 702870 & 29000 & 120000 & 185000 & 247468.7 & 298000 & 1700000 & 6748 \\ 
  pricem2 & 696064 & 465 & 1363.636 & 2000 & 2299.238 & 2941.176 & 7900 & 13554 \\ 
  visits & 702601 & 94 & 707 & 1461 & 2383.044 & 2961 & 20721 & 7017 \\ 
  leads & 706025 & 0 & 0 & 1 & 3.45574 & 4 & 52 & 3593 \\ 
   \hline
\hline
\caption{Variables of type \texttt{Date}. If the end date is missing, it means that
at least one of the ads associated to the housing unit is still visible by the latest
available weekly snapshot.} 
\label{tab:summstatcleaneddate}
\end{longtable}
\endgroup



==> tables/summary-statistics-diffrel-price.tex <==



==> tables/summary-statistics-factor-OMI-infolocIstat.tex <==
% latex table generated in R 3.0.3 by xtable 1.7-3 package
% Mon Sep  5 08:47:19 2016
{\footnotesize
\begin{longtable}{llrr}
 \textbf{Variable} & \textbf{Levels} & $\mathbf{n}$ & $\mathbf{\%}$ \\ 
  \hline
Zona\_OMI & ABANO TERME - Zona OMI B1 & 1 & 0.0 \\ 
   & ABANO TERME - Zona OMI B2 & 1 & 0.0 \\ 
   & ABANO TERME - Zona OMI D3 & 1 & 0.0 \\ 
   & ABANO TERME - Zona OMI E1 & 1 & 0.0 \\ 
   & ABANO TERME - Zona OMI E2 & 1 & 0.0 \\ 
   & ABANO TERME - Zona OMI R1 & 1 & 0.0 \\ 
   & ABANO TERME - Zona OMI R2 & 1 & 0.0 \\ 
   & ABBADIA CERRETO - Zona OMI B & 1 & 0.0 \\ 
   & ABBADIA CERRETO - Zona OMI R1 & 1 & 0.0 \\ 
   & ABBADIA LARIANA - Zona OMI B2 & 1 & 0.0 \\ 
   & (Others) & 27160 & 100.0 \\ 
   \hline
 & all & 27170 & 100.0 \\ 
   \hline
\hline
Area\_territoriale & NORD-OVEST & 8864 & 32.6 \\ 
   & SUD & 6181 & 22.8 \\ 
   & NORD-EST & 4787 & 17.6 \\ 
   & CENTRO & 4088 & 15.1 \\ 
   & ISOLE & 2658 & 9.8 \\ 
   & missing & 592 & 2.2 \\ 
   \hline
 & all & 27170 & 100.0 \\ 
   \hline
\hline
Regione & LOMBARDIA & 4279 & 15.8 \\ 
   & PIEMONTE & 3266 & 12.0 \\ 
   & VENETO & 2120 & 7.8 \\ 
   & CAMPANIA & 2061 & 7.6 \\ 
   & SICILIA & 1624 & 6.0 \\ 
   & LAZIO & 1458 & 5.4 \\ 
   & TOSCANA & 1359 & 5.0 \\ 
   & EMILIA-ROMAGNA & 1356 & 5.0 \\ 
   & CALABRIA & 1335 & 4.9 \\ 
   & TRENTINO-ALTO ADIGE & 1224 & 4.5 \\ 
   & (Others) & 7085 & 26.1 \\ 
   & missing & 3 & 0.0 \\ 
   \hline
 & all & 27170 & 100.0 \\ 
   \hline
\hline
Prov & Torino & 948 & 3.5 \\ 
   & Trento & 743 & 2.7 \\ 
   & Cuneo & 687 & 2.5 \\ 
   & Brescia & 663 & 2.4 \\ 
   & Roma & 596 & 2.2 \\ 
   & Salerno & 571 & 2.1 \\ 
   & Bergamo & 563 & 2.1 \\ 
   & Varese & 510 & 1.9 \\ 
   & Napoli & 506 & 1.9 \\ 
   & Bolzano/Bozen & 455 & 1.7 \\ 
   & (Others) & 20897 & 76.9 \\ 
   & missing & 31 & 0.1 \\ 
   \hline
 & all & 27170 & 100.0 \\ 
   \hline
\hline
Comune\_descrizione & Roma & 233 & 0.9 \\ 
   & Genova & 81 & 0.3 \\ 
   & Napoli & 65 & 0.2 \\ 
   & Palermo & 51 & 0.2 \\ 
   & Milano & 41 & 0.1 \\ 
   & Torino & 41 & 0.1 \\ 
   & Trento & 38 & 0.1 \\ 
   & Venezia & 36 & 0.1 \\ 
   & Bari & 35 & 0.1 \\ 
   & Bologna & 34 & 0.1 \\ 
   & (Others) & 26484 & 97.5 \\ 
   & missing & 31 & 0.1 \\ 
   \hline
 & all & 27170 & 100.0 \\ 
   \hline
\hline
\hline
\caption{Categorical OMI variables in OMI microzones, correcting with Istat information} 
\label{tab:summstatcatOMIinfolocIstat}
\end{longtable}
}



==> tables/summary-statistics-numeric-Istat-OMI.tex <==
% latex table generated in R 3.0.3 by xtable 1.7-3 package
% Tue Sep  6 13:21:03 2016
{\footnotesize
\begin{longtable}{lrrrrrrrr}
 Variable & N & Min. & 1st Qu. & Median & Mean & 3rd Qu. & Max. & NA \\ 
  \hline
Ptot & 27158 &  0.00 &    212.00 &     707.00 &     2076.75 &     2062.75 &    131160.00 &    12 \\ 
  P0.14 & 26907 &  0.00 &      0.11 &       0.13 &        0.13 &        0.15 &         0.60 &   263 \\ 
  P15.24 & 26907 &  0.00 &      0.08 &       0.10 &        0.10 &        0.11 &         0.99 &   263 \\ 
  P25.34 & 26907 &  0.00 &      0.10 &       0.12 &        0.12 &        0.13 &         0.98 &   263 \\ 
  P35.54 & 26907 &  0.00 &      0.29 &       0.31 &        0.31 &        0.33 &         1.00 &   263 \\ 
  P55.64 & 26907 &  0.00 &      0.11 &       0.13 &        0.13 &        0.14 &         1.00 &   263 \\ 
  Ped\_degree & 26907 &  0.00 &      0.06 &       0.08 &        0.09 &        0.10 &         1.00 &   263 \\ 
  Ped\_diploma & 26907 &  0.00 &      0.57 &       0.60 &        0.60 &        0.63 &         1.00 &   263 \\ 
  Pocc\_labforce & 26907 &  0.00 &      0.46 &       0.51 &        0.51 &        0.56 &         1.00 &   263 \\ 
  Pocc\_unemp & 26906 &  0.00 &      0.04 &       0.06 &        0.07 &        0.09 &         0.97 &   264 \\ 
  Pcommut & 26907 &  0.00 &      0.16 &       0.25 &        0.24 &        0.33 &         1.00 &   263 \\ 
  Pforeign & 26907 &  0.00 &      0.02 &       0.05 &        0.06 &        0.09 &         0.99 &   263 \\ 
  PFtot & 27158 &  0.00 &     93.00 &     297.00 &      861.00 &      844.75 &     63766.00 &    12 \\ 
  PF1 & 26907 &  0.00 &      0.25 &       0.31 &        0.33 &        0.38 &         1.00 &   263 \\ 
  PF2 & 26907 &  0.00 &      0.23 &       0.26 &        0.26 &        0.29 &         1.00 &   263 \\ 
  PF3 & 26907 &  0.00 &      0.16 &       0.20 &        0.19 &        0.22 &         1.00 &   263 \\ 
  PF4 & 26907 &  0.00 &      0.12 &       0.16 &        0.16 &        0.19 &         1.00 &   263 \\ 
  PF5 & 26907 &  0.00 &      0.03 &       0.04 &        0.04 &        0.06 &         1.00 &   263 \\ 
  Htot & 27158 &  0.00 &     91.00 &     239.00 &      417.29 &      521.00 &     16649.00 &    12 \\ 
  Htot\_dwell & 27158 &  0.00 &    171.00 &     490.00 &     1170.41 &     1254.00 &     71465.00 &    12 \\ 
  Hprimary & 26891 &  0.00 &      0.58 &       0.77 &        0.71 &        0.88 &         1.00 &   279 \\ 
  Hrent & 26876 &  0.00 &      0.07 &       0.11 &        0.13 &        0.17 &         1.00 &   294 \\ 
  Hown & 26876 &  0.00 &      0.70 &       0.76 &        0.75 &        0.81 &         1.00 &   294 \\ 
  Hage\_1918 & 26892 &  0.00 &      0.04 &       0.12 &        0.20 &        0.29 &         1.00 &   278 \\ 
  Hage\_1919\_1945 & 26892 &  0.00 &      0.04 &       0.08 &        0.11 &        0.16 &         1.00 &   278 \\ 
  Hage\_1946\_1960 & 26892 &  0.00 &      0.05 &       0.11 &        0.13 &        0.17 &         1.00 &   278 \\ 
  Hage\_1961\_1970 & 26892 &  0.00 &      0.08 &       0.14 &        0.15 &        0.20 &         0.99 &   278 \\ 
  Hage\_1971\_1980 & 26892 &  0.00 &      0.08 &       0.14 &        0.16 &        0.21 &         1.00 &   278 \\ 
  Hage\_1981\_1990 & 26892 &  0.00 &      0.04 &       0.09 &        0.11 &        0.15 &         1.00 &   278 \\ 
  Hage\_1991\_2000 & 26892 &  0.00 &      0.02 &       0.06 &        0.07 &        0.10 &         0.98 &   278 \\ 
  Hage\_2001\_2005 & 26892 &  0.00 &      0.01 &       0.03 &        0.04 &        0.05 &         1.00 &   278 \\ 
  Hage\_2006\_ & 26892 &  0.00 &      0.00 &       0.02 &        0.03 &        0.04 &         0.99 &   278 \\ 
  Hfloor\_1 & 26892 &  0.00 &      0.05 &       0.10 &        0.15 &        0.19 &         1.00 &   278 \\ 
  Hfloor\_2 & 26892 &  0.00 &      0.37 &       0.52 &        0.51 &        0.65 &         1.00 &   278 \\ 
  Hfloor\_3 & 26892 &  0.00 &      0.12 &       0.24 &        0.25 &        0.36 &         1.00 &   278 \\ 
  Hfloor\_4\_ & 26892 &  0.00 &      0.01 &       0.03 &        0.09 &        0.10 &         0.96 &   278 \\ 
  Hunit\_1 & 26892 &  0.00 &      0.36 &       0.53 &        0.53 &        0.70 &         1.00 &   278 \\ 
  Hunit\_2 & 26892 &  0.00 &      0.16 &       0.24 &        0.23 &        0.30 &         1.00 &   278 \\ 
  Hunit\_3\_4 & 26892 &  0.00 &      0.06 &       0.12 &        0.13 &        0.18 &         1.00 &   278 \\ 
  Hunit\_5\_8 & 26892 &  0.00 &      0.01 &       0.04 &        0.06 &        0.09 &         0.97 &   278 \\ 
  Hunit\_9\_15 & 26892 &  0.00 &      0.00 &       0.01 &        0.03 &        0.03 &         0.92 &   278 \\ 
  Hunit\_16\_ & 26892 &  0.00 &      0.00 &       0.00 &        0.02 &        0.01 &         1.00 &   278 \\ 
  Hpreserv\_optimal & 26892 &  0.00 &      0.16 &       0.29 &        0.32 &        0.45 &         1.00 &   278 \\ 
  Hpreserv\_good & 26892 &  0.00 &      0.40 &       0.51 &        0.51 &        0.62 &         1.00 &   278 \\ 
  Hpreserv\_mediocre & 26892 &  0.00 &      0.07 &       0.13 &        0.15 &        0.20 &         1.00 &   278 \\ 
  Hpreserv\_terrible & 26892 &  0.00 &      0.00 &       0.01 &        0.02 &        0.02 &         0.99 &   278 \\ 
  Entropy & 26892 &  0.00 &      4.23 &       4.74 &        4.64 &        5.17 &         6.24 &   278 \\ 
  distances &  2159 & 11.57 &   1576.09 &    3426.35 &     4899.03 &     6611.22 &     54457.55 & 25011 \\ 
  area & 27170 &  0.00 &      0.00 &       0.00 &        0.00 &        0.00 &         0.07 &     0 \\ 
  Hdensity & 27158 &  0.00 & 335674.07 & 5109759.42 & 14608791.03 & 17190600.84 & 401771935.40 &    12 \\ 
  supply &   881 &  0.00 &      0.02 &       0.03 &        0.03 &        0.04 &         0.50 & 26289 \\ 
  demand &   882 &  9.00 &    642.92 &     909.38 &     1045.02 &     1243.43 &      6676.00 & 26288 \\ 
  \hline
\caption{Numeric Istat variables in OMI microzones} 
\label{tab:summstatnumericIstatOMI}
\end{longtable}
}

==> tables/summary-statistics-numeric.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Thu Sep 14 22:00:01 2017
\begingroup\footnotesize
\begin{longtable}{p{4cm}rrrrrrrr}
 Variable & N & Min. & 1st Qu. & Median & Mean & 3rd Qu. & Max. & NA \\ 
  \hline
Floor area & 647,223 &    27.0 &     70.0 &     93.0 &    108.9 &    130 &     550.0 &  6,276 \\ 
  Number of rooms & 630,220 &     1.0 &      3.0 &      3.0 &      3.3 &      4 &       5.0 & 23,279 \\ 
  Number of bathrooms & 640,468 &     1.0 &      1.0 &      1.0 &      1.5 &      2 &       3.0 & 13,031 \\ 
  Ads that refer to the same housing unit & 653,499 &     1.0 &      1.0 &      1.0 &      1.6 &      2 &     105.0 &     0 \\ 
  Time on market & 298,843 &     8.0 &    92.0 &    189.0 &    268.4 &    360 &    1,512.0 &  354,656 \\ 
  Price & 647,330 & 25,000 & 128,000 & 196,000 & 269,900 & 320,000 & 2,120,000 &  6,169 \\ 
  Price per m2 & 640,752 &   393.3 &   1,467.2 &   2,142.9 &   2,466.5 &   3,125 &    9,166.7 & 12,747 \\ 
  Visits on ads that refer to the same housing unit & 646,989 &    43.0 &    487.0 &   1,102.0 &   1,834.8 &   2,340 &   15,435.0 &  6,510 \\ 
  Favorites on ads that refer to the same housing unit & 649,970 &     0.0 &      0.0 &      1.0 &      2.5 &      3 &      39.0 &  3,529 \\ 
  \hline
\caption{Numeric variables. In the cases of floor area, time on market, price, price per m2, visits and favorites we remove the upper and lower 0.5\% of the distribution. Extreme values are often outliers due to misreporting by the real estate agents. The time on market is calculated only for the housing units that have disappeared from the dataset. Note also that the number of rooms is limited to ``5 or more''.} 
\label{tab:summstatcleanednumeric}
\end{longtable}
\endgroup

==> tables/summary-statistics-numerical.tex <==
% latex table generated in R 3.4.1 by xtable 1.8-2 package
% Wed Mar 27 19:42:35 2019
\begingroup\footnotesize
\begin{longtable}{lrrrrrrrr}
 Variable & N & Min. & 1st Qu. & Median & Mean & 3rd Qu. & Max. & NA \\ 
  \hline
Floor area & 703075 &    27 &     70.0 &     93 &    107.8 &    125.0 &     500 &  6543 \\ 
  Number of rooms & 689219 &     1 &      2.0 &      3 &      3.3 &      4.0 &       5 & 20399 \\ 
  Number of bathrooms & 698000 &     1 &      1.0 &      1 &      1.5 &      2.0 &       3 & 11618 \\ 
  Number of duplicates & 709618 &     1 &      1.0 &      1 &      1.6 &      2.0 &      99 &     0 \\ 
  Time on market & 703632 &    15 &     74.0 &    158 &    240.4 &    300.0 &    1733 &  5986 \\ 
  Price & 702870 & 29000 & 120000.0 & 185000 & 247468.7 & 298000.0 & 1700000 &  6748 \\ 
  Price per m2 & 696064 &   465 &   1363.6 &   2000 &   2299.2 &   2941.2 &    7900 & 13554 \\ 
  Total clicks & 702601 &    94 &    707.0 &   1461 &   2383.0 &   2961.0 &   20721 &  7017 \\ 
  Total contacts & 706025 &     0 &      0.0 &      1 &      3.5 &      4.0 &      52 &  3593 \\ 
  \hline
\caption{Numeric variables. In the cases of floor area, time on market, price, price per m2, clicks and
contacts we remove the upper and lower 0.5% of the distribution: Extreme values are often outliers due
to misreporting by the real estate agents. The time on market is calculated only for housing units
that have disappeared from the dataset. Note also that above four rooms, all units are 
registered as having ''five or more`` rooms.} 
\label{tab:summstatcleanednumeric}
\end{longtable}
\endgroup


==> tables/table_ads_dwell_cities.tex <==
% latex table generated in R 3.5.3 by xtable 1.8-3 package
% Sun Feb  9 20:37:33 2020
\begin{table}[ht]
\centering
\begin{tabular}{lccc}
  \hline
city\_istat\_code & n\_ads & n\_id & share \\ 
  \hline
58091 & 1 & 189138 & 2 \\ 
  15146 & 1 & 98253 & 2 \\ 
  1272 & 1 & 68489 & 1 \\ 
  10025 & 1 & 40659 & 1 \\ 
  63049 & 1 & 31555 & 1 \\ 
  48017 & 1 & 28896 & 2 \\ 
  82053 & 1 & 25702 & 1 \\ 
  37006 & 1 & 24966 & 2 \\ 
   \hline
\end{tabular}
\caption{Number of ads and houses in the main cities} 
\label{table:ads_dwell_cities}
\end{table}


==> tables/table_dupl_determinants.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Thu, Apr 04, 2019 - 04:58:42 PM
\begin{table}[!htbp] \centering 
\footnotesize
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{$DUPLIC$} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex]  
$DEMAND$ & $-$1.050$^{***}$ & 0.350$^{***}$ \\ 
$RELPRICE$ & $-$0.035$^{*}$ & 0.966$^{*}$ \\ 
$OVERVAL$ & $-$0.690$^{***}$ & 0.502$^{***}$ \\
Fixed effects & City & City \\ 
Temporal dummies & Quarter & Quarter \\
\hline \\[-1.8ex] 
Observations & 1,547,919 & 1,547,919 \\ 
\hline 
\hline \\[-1.8ex] 
\multicolumn{3}{l}{Column (1) are the coefficients of the logit estimation. Column (2) is the log-odd ratio.} \\ 
\end{tabular} 
\caption{Determinants of duplicated advertisements. \mrc{Toglierei le stelline e metterei gli errori standard.}} 
  \label{table:table_dupl_determinants} 
\end{table} 


==> tables/tightness_predictor_controls_Pitminus1_quarter_severalOMI.tex <==
% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: gio, set 14, 2017 - 00:40:23
% Requires LaTeX packages: dcolumn 
\begin{table}[!htbp] \centering 
  \caption{Tightness predictive power} 
  \label{tab:tightnesspredictor} 
\begin{tabular}{@{\extracolsep{-100pt}}lD{.}{.}{-3} } 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & \multicolumn{1}{c}{Price per m2 (t) [log]} \\ 
\hline \\[-1.8ex] 
 Price per m2 (t-1) [log] ($\delta_0$) & 0.506^{***}$ $(0.010) \\ 
 Tightness (t-1) [log] ($\beta_1$) & 0.044^{***}$ $(0.013) \\ 
 Tightness (t-2) [log] ($\beta_2$) & 0.048^{***}$ $(0.013) \\ 
 Constant ($\alpha$) & 3.211^{***}$ $(0.120) \\ 
 \hline \\[-1.8ex] 
Observations & \multicolumn{1}{c}{6,288} \\ 
R$^{2}$ & \multicolumn{1}{c}{0.811} \\ 
Adjusted R$^{2}$ & \multicolumn{1}{c}{0.807} \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
 & \multicolumn{1}{r}{City and quarter dummies. Other controls
          include OMI area characteristics.} \\ 
 & \multicolumn{1}{r}{Data are aggregated over OMI areas and 
                                                   quarters, from 2016Q1 to 2017Q2.} \\ 
\end{tabular} 
\end{table} 

